Meta-Learning for Domain Generalization in Semantic Parsing

The importance of building semantic parsers which can be applied to new domains and generate programs unseen at training has long been acknowledged, and datasets testing out-of-domain performance are becoming increasingly available. However, little or no attention has been devoted to learning algorithms or objectives which promote domain generalization, with virtually all existing approaches relying on standard supervised learning. In this work, we use a meta-learning framework which targets zero-shot domain generalization for semantic parsing. We apply a model-agnostic training algorithm that simulates zero-shot parsing by constructing virtual train and test sets from disjoint domains. The learning objective capitalizes on the intuition that gradient steps that improve source-domain performance should also improve target-domain performance, thus encouraging a parser to generalize to unseen target domains. Experimental results on the (English) Spider and Chinese Spider datasets show that the meta-learning objective significantly boosts the performance of a baseline parser.

==> tables/ch_spider_main_results_dev.tex <==
\begin{table}[t!]
    \centering
    \begin{adjustbox}{max width=\columnwidth, center}
        \begin{tabular}{lc}
            \toprule
            \bfseries Model & \bfseries Set Match \\
            \midrule
            SyntaxSQLNet \citep{yu-etal-2018-syntaxsqlnet} & 16.4 \\
            \textbf{Our Models} \\
            \quad    Base Parser & 31.0 \\ 
            \quad    Base Parser + DG-MAML & \textbf{35.5} \\ 
            \midrule
            \textit{With Pratrained Representations:} \\
            RYANSQL + M-BERT \citep{choi2020ryansql} & 41.3  \\
            \textbf{Our Models} \\
            \quad  Base Parser + M-BERT & 47.0 \\ 
            \quad  Base Parser + M-BERT + DG-MAML & \textbf{50.1} \\ 
            \bottomrule
        \end{tabular}
    \end{adjustbox}
    \caption{Set match accuracy (\%) on the development Chinese Spider. M-BERT: Multiligual-BERT.}
    \label{table:main-results}
    \vspace{-3mm}
\end{table}

==> tables/en_spider_main_results_dev.tex <==
\begin{table}[t]
    \centering
    \begin{adjustbox}{max width=\columnwidth, center}
        \begin{tabular}{lc}
            \toprule
            %\bfseries Model & \bfseries SM & \bfseries EXE \\
            \bfseries Model & \bfseries Set Match \\
            \midrule
            SyntaxSQLNet \citep{yu-etal-2018-syntaxsqlnet} & 18.9 \\
            Global-GNN \citep{bogin-etal-2019-global} & 52.7 \\
            IRNet \citep{guo-etal-2019-towards} & 55.4  \\
            RAT-SQL \citep{wang2019rat} & \textbf{62.7}  \\
            \textbf{Our Models} \\
            \quad    Base Parser & 56.4 \\ 
            \quad    Base Parser + DG-MAML & 58.5   \\ 
            \midrule
            \textit{With Pratrained Representations:} \\
            RAT-SQL + BERT-large \citep{wang2019rat} & 69.7  \\
            RYANSQL + BERT-large \citep{choi2020ryansql} & \textbf{70.6}  \\
            IRNet + BERT-base \citep{guo-etal-2019-towards} & 61.9  \\
            \textbf{Our Models} \\
            \quad  Base Parser + BERT-base & 66.8 \\ 
            \quad  Base Parser + BERT-base + DG-MAML & 68.9  \\ 
            \bottomrule
        \end{tabular}
    \end{adjustbox}
    \caption{Set match accuracy (\%) on the development of Spider.}
    \label{table:en-main-results}
    \vspace{-3mm}
\end{table}

==> tables/spider_difficulty.tex <==
\begin{table*}[t!]
    \begin{subtable}[t]{0.5\textwidth}
        \centering
        \small
        \begin{tabular}{lrrrrr}
            \toprule
            \bfseries Split  & \bfseries Easy & \bfseries Medium & \bfseries Hard & \bfseries Extra Hard & \bfseries All \\
            \midrule
            \multicolumn{5}{l}{\textit{Base Parser}} \\
            %\cmidrule{1-1}
            \bfseries Dev & 56.8 & 40.2 & 30.5 & 22.9 & 39.7 \\
            \bfseries Test & 56.3  & 34.8  & 28.9  & 13.5  & 34.6  \\
            \midrule
            \multicolumn{5}{l}{\textit{Base Parser + DG-MAML}} \\
            %\cmidrule{1-1}
            \bfseries Dev & 61.6  & 47.3 & 32.8 & 21.8 & 44.1 \\
            \bfseries Test & 59.7  & 41.3 & 32.2 & 21.0 & 39.9  \\
            \bottomrule
        \end{tabular}
        \caption{Accuracy(\%) on the Spider dataset.}
        \label{table:en_bydifficulty}
    \end{subtable}
    \hfill
    \begin{subtable}[t]{0.5\textwidth}
        \centering
        \small
        \begin{tabular}{lrrrrr}
            \toprule
            \bfseries Split  & \bfseries Easy & \bfseries Medium & \bfseries Hard & \bfseries Extra Hard & \bfseries All \\
            \midrule
            \multicolumn{5}{l}{\textit{Base Parser}} \\
            %\cmidrule{1-1}
            \bfseries Dev & 46.0 & 30.5 & 24.7 & 17.1 & 31.0   \\
            \bfseries Test & 41.2  & 20.0  & 16.8 & 14.3  & 23.0 \\
            \midrule
            \multicolumn{5}{l}{\textit{Base Parser + DG-MAML}} \\
            %\cmidrule{1-1}
            \bfseries Dev & 52.8   & 34.1 & 28.7 & 20.6 & 35.5 \\
            \bfseries Test & 42.9  & 28.9 & 17.9 & 12.4 & 26.8  \\
            \bottomrule
        \end{tabular}
        \caption{Accuracy (\%) on the Chinese Spider dataset.}
        \label{table:ch_bydifficulty}
    \end{subtable}
    \caption{Comparison of performance by difficulty as defined by \citet{yu-etal-2018-spider}.}
    \label{table:acc_bydifficulty}
\end{table*}

